A Simple but Effective Approach to Improve Structured Language Model Output for Information Extraction

Large language models (LLMs) have demonstrated impressive abilities in generating unstructured natural language according to instructions. However, their performance can be inconsistent when tasked with producing text that adheres to specific structured formats, which is crucial in applications like named entity recognition (NER) or relation extraction (RE). To address this issue, this paper introduces an efficient method, G&O, to enhance their structured text generation capabilities. It breaks the generation into a two-step pipeline: initially, LLMs generate answers in natural language as intermediate responses. Subsequently, LLMs are asked to organize the output into the desired structure, using the intermediate responses as context. G&O effectively separates the generation of content from the structuring process, reducing the pressure of completing two orthogonal tasks simultaneously. Tested on zero-shot NER and RE, the results indicate a significant improvement in LLM performance with minimal additional efforts. This straightforward and adaptable prompting technique can also be combined with other strategies, like self-consistency, to further elevate LLM capabilities in various structured text generation tasks.

==> sections/2.theory.tex <==
\section{Theory}
\label{sec:theory}


As probabilistic models pre-trained on causal inference tasks with unstructured text, LLMs have not demonstrated a concrete sign of being able to reason intrinsically \citep{Huang.2023.LLM.self.correct, Valmeekam.2023.self.critiquing.plans, Stechly.2023.iterative.prompting, Li.2023.Minesweeper}.
Their generation performance largely relies on the alignment between the pre-training corpus and the input instruction \citep{Xie.2022.in.context.learning, Min.2022.rethinking.demonstrations, Gudibande.2023.the.false.promise}.
Specifically, \citet{Xie.2022.in.context.learning} demonstrate that LLMs present in-context learning ability when they infer coherent latent concept flows within both pre-training and test instruction data, even though the latent spaces themselves are explicitly aligned.
Although irrelevant to in-context learning, we borrow the ``concept transition'' concept from \citet{Xie.2022.in.context.learning} for a more intuitive but less rigorous explanation of the structuring prompting scenario.

Instead of individual tokens, natural language can also be considered as a flow of latent concepts, whose transition can be modeled by a Markov chain.
Therefore, the token inner dependencies of a length-$T$ sequence $\x=[x_1, \dots, x_T], \forall x_i\in\tokens$ can be simplified and modeled by a (high-order) hidden Markov model (HMM) with $T$ latent states $\h=[h_1, \dots, h_T]$, where each state $h_t$ represents a latent concept:\footnote{A more rigorous analogy is the hidden semi-Markov model (HSMM, \citealp{Yu.2010.HSMM}), where each latent concept spans multiple observed tokens. However, we omit the duration modeling for simplicity.}
The observation probability is defined as
\begin{equation*}
  \begin{aligned}
    p(\x|\btheta) = \int_{\h} p(\x|\h, \btheta) p(\h|\btheta) d\h.
  \end{aligned}
\end{equation*}
$\btheta$ denotes the model parameters that simulate the transition and emission probabilities of HMM: $\btheta=\{\trans\in\real^{|\concept|\times |\concept|}, \emiss\in\real^{|\concept|\times|\tokens|}\}$, where $\concept$ is the set of all latent concepts with \emph{unknown} size.
From this perspective, the LLM inference step can be considered as a process of sampling the most likely latent concept sequence $\h_{\rm pred}$ according to the fitted transition matrix $\trans$ and the history latent states $\h_{\rm prompt}$ inferred from the prompt tokens $\x_{\rm prompt}$, and then generating the tokens $\x_{\rm pred}$ according to the emission probabilities $\emiss$.

Such a setup exposes the potential issue of concept transition mismatch in a prompt, which could be a factor in the formatting failure.
Specifically, most of the written material presents a relatively fixed logic flow, making the transition matrix $\trans$ sparse.
When applied to inference, $\trans$ can help LLMs generate highly convincing tokens $\x_{\rm pred}$ that follow the logic flow $\h_{\rm pred}$, if the prompting text $\x_{\rm prompt}$ indicates a valid sequence of $\h_{\rm prompt}$.
In other words, LLMs generate well when the latent concept transition in the prompt is in the pre-training domain.

Things become trickier when $\x_{\rm prompt}$ leads to an abnormal flow of concepts.
For example, according to $\emiss$, sentence $\x_1$ leads to $\h_1$, and the subsequent sentence $\x_2$ leads to $\h_2$.
However, as $\x_1$ and $\x_2$ are rarely co-occurred in the pre-training corpus, the transition $\trans_{\h_1\to \h_2}$ is close to 0.
Usually, 0 transition represents the end of the previous latent concept group and the start of a new one, as signaled by the ``delimiter'' in \citep{Xie.2022.in.context.learning}.
But LLM prompting is mostly designed to handle one task.
The disruption in the continuous logic flow could result in a flat distribution of the predicted latent concepts $\h_{\rm pred}$, \ie, $p(\h_{\rm pref})$ has a large entropy, which inevitably results in low $\h_{\rm pred}$ sampling quality and a sub-optimal $\x_{\rm pred}$.

\begin{theorem}
  \label{thm:1}
  Given a prompt $\x_{\rm prompt}$, the probability of a well-formed (but not necessarily correct) output $\x_{\rm pred}$ is proportional to the product of the transition probabilities of the latent concept sequence $p(\text{well-formed } \x_{\rm pred})\propto \prod_{i=2}^{l}\trans_{h_{i-1}, h{i}}$, where $h_i$ is the $i$-th element in sequence $\h_{\rm prompt}$ and $l$ is the length of the sequence.
\end{theorem}

With \cref{thm:1}, we can inspect language model fine-tuning from another perspective: it increases certain elements in $\trans$ such that there are less or no 0 valleys in the latent semantic transition path.
Instruction tuning mainly focuses on ``smoothing'' the transition within the prompt, whereas task-specific fine-tuning such as CoT tuning \citep{Wei.2022.chain.of.thought} also aims to update the concept transitions within the predicted text sequence.


==> sections/3.ie.tex <==
\section{Analysis for Information Extraction}
\label{sec:ie}

\subsection{Problem}

Generally, the simple IE instructions such as ``\textit{please identify the `person' entities}'' followed by the context are commonly seen in LLMs' training materials, presenting a set of greater-than-zero inner transitions within the instruction semantics.
In the mathematical expression, we have $\trans_{\h_{\rm instr-IE}\to \h_{\rm context}}=c_1>0$ and $\trans_{\h_{\rm context}\to \h_{\rm pred-free}}=c_2>0$ where $c_1$ and $c_2$ are not close to 0.
However, when we require structured output, the instruction becomes the composition of two parts: the IE part $\x_{\rm instr-IE}$ and the formatting part $\x_{\rm instr-format}$, \eg ``\textit{output as a list}'', which are diagonal in semantics.
The diagonality poses a close-to-0 transition between the two parts, \ie, $\trans_{\h_{\rm instr-IE}\to \h_{\rm instr-format}}\approx 0$, which, according to \cref{thm:1}, results in a low probability of well-formed output: $\x_{\rm pred}$ is likely to either be well-structured but incorrect or randomly-formatted.

\subsection{Solution}

Since we are not able to update the parameters of GPT models to increase the desired transition probabilities, we take the only other straightforward solution: removing the concept link that causes the 0 transitions and placing it in a position where the transition to and from the latent concept is no longer 0.
Recall that the transition matrix $\trans$ is defined by model parameters $\btheta$, which is highly dependent on the training material in unstructured language.
Therefore, an intuitive way is leveraging the multi-round conversation scheme of GPTs.
In the first round, we generate the free-formed IE results $\x_{\rm pred-free}$ using only IE instructions $\x_{\rm instr-IE}$.
Then, we use the generated $\x_{\rm pred-free}$ as the new context, with which we apply the formatting instruction $\x_{\rm instr-format}$ to generate the final structured output $\x_{\rm pred}$.
Considering that the formatting operation is not rare, we can safely guarantee that the inter-transition $\trans_{\h_{\rm pred-free}\to \h_{\rm instr-format}}$ and inner-transition $\trans_{h_i\to h_{i+1}}, h_i\in\{\h_{\rm instr-format}\}$ are not close to 0.


==> sections/tables/s1.ner.result.tex <==
\begin{table*}[ht] \small
  \centering
  \begin{tabular}{lllllllll}
  \hline
  & \multicolumn{2}{c}{CoNLL 2003} & \multicolumn{2}{c}{BC5CDR} & \multicolumn{2}{c}{NCBI Disease} & \multicolumn{2}{c}{PolyIE} \\ 
  & partial & full & partial & full & partial & full & partial & full \\ 
  \hline
  GPT 3.5 & & & & & & & & \\
  aeio & 0.5370 (0.6819 / 0.4429) & 0.4965 (0.6323 / 0.4088) & 0.6199 (0.8254 / 0.4963) & 0.5058 (0.6794 / 0.4028) & & & 0.1300 (0.7440 / 0.0712) & 0.0935 (0.5383 / 0.0512) \\
  one\_step & 0.4741 (0.4070 / 0.5678) & 0.4477 (0.3850 / 0.5349) & 0.7030 (0.6632 / 0.7479) & 0.6041 (0.5720 / 0.6401) & 0.6500 (0.6175 / 0.6860) & 0.5131 (0.4851 / 0.5445) & 0.4669 (0.4253 / 0.5177) & 0.3207 (0.2936 / 0.3533) \\
  ino & 0.6569 (0.6027 / 0.7219) & 0.6192 (0.5695 / 0.6784) & 0.7610 (0.7835 / 0.7398) & 0.6079 (0.6334 / 0.5845) & 0.6935 (0.8458 / 0.5877) & 0.5047 (0.6278 / 0.4220) & 0.5449 (0.5830 / 0.5115) & 0.3823 (0.4117 / 0.3569) \\
  ino-cr & 0.6775 (0.6386 / 0.7213) & 0.6394 (0.6043 / 0.6788) & 0.7724 (0.7954 / 0.7506) & 0.6186 (0.6447 / 0.5946) & - & - & 0.6011 (0.6723 / 0.5572) & 0.4236 (0.4685 / 0.3866) \\
  bert & 0.7175 (0.6496 / 0.8012) & 0.6800 (0.6161 / 0.7585) & 0.7949 (0.8166 / 0.7743) & 0.6838 (0.7068 / 0.6622) & 0.7703 (0.8822 / 0.6837) & 0.5507 (0.6356 / 0.4859) & 0.7608 (0.7044 / 0.8270) & 0.5533 (0.5034 / 0.6141) \\
  no-purify & 0.7003 (0.6482 / 0.7616) & 0.6436 (0.5992 / 0.6950) & 0.7421 (0.7153 / 0.7712) & 0.5861 (0.5699 / 0.6032) & 0.6475 (0.6775 / 0.6200) & 0.4541 (0.4886 / 0.4242) & 0.5103 (0.5036 / 0.5173) & 0.3421 (0.3396 / 0.3448) \\
  \hline
  \end{tabular}
  \caption{Your table caption here.}
\end{table*}

